S3: Side-Channel Attack on Stylus Pencil through Sensors

With smart devices being an essential part of our everyday lives, unsupervised access to the mobile sensors' data can result in a multitude of side-channel attacks. In this paper, we study potential data leaks from Apple Pencil (2nd generation) supported by the Apple iPad Pro, the latest stylus pen which attaches to the iPad body magnetically for charging. We observe that the Pencil's body affects the magnetic readings sensed by the iPad's magnetometer when a user is using the Pencil. Therefore, we ask: Can we infer what a user is writing on the iPad screen with the Apple Pencil, given access to only the iPad's motion sensors' data? To answer this question, we present Side-channel attack on Stylus pencil through Sensors (S3), a system that identifies what a user is writing from motion sensor readings. We first use the sharp fluctuations in the motion sensors' data to determine when a user is writing on the iPad. We then introduce a high-dimensional particle filter to track the location and orientation of the Pencil during usage. Lastly, to guide particles, we build the Pencil's magnetic map serving as a bridge between the measured magnetic data and the Pencil location and orientation. We evaluate S3 with 10 subjects and demonstrate that we correctly identify 93.9%, 96%, 97.9%, and 93.33% of the letters, numbers, shapes, and words by only having access to the motion sensors' data.

==> miscellaneous/attack_model_old.tex <==
\section{Threat Model}
\label{sec:threat_model}
Given the huge popularity of tablet devices, such as iPad, side-channel attacks on these devices compromising users' privacy have a huge impact on user security.
%
%Mobile operating systems allowing access to motion sensor's data to all applications by default without requiring any permissions have facilitated such attacks.
%
Due to the loophole in mobile operating systems' access control definitions, any seemingly useful application installed via application store such as Apple's AppStore can record the motion sensors' data by default, without requiring any user permission.
%-
While our proposed attack of inferring information about what the user is writing from motion sensors' data can be a threat for any mobile device that supports a stylus pen with embedded magnets, in this paper, we only focus on Apple's iPad and Pencil (2nd generation) to demonstrate proof of concept.

In our threat model, we assume that the attacker has installed a malicious application on the victim's device.
%
This application does not require any privileged access from the system or additional user permissions, apart from access to the Internet, which is granted by default. 
%
The application also does not have any information about other running applications and
does not have access to system resources. 
%Therefore, attacker's malicious code can be hidden in any application which victims are likely to install. 
%
Starting from iOS 5, execution of any iOS application is suspended shortly after being moved to the background.
%
Moreover, iOS does not allow applications to stay active in the background for an arbitrary amount of time.
%
However, an application can stay active in the background if it is performing specific actions like playing audio, receiving updates from a server or using location services. 
%
Therefore the attacker's application can masquerade as a benign fitness activity tracker or a music player (playing inaudible sound) to stay active in the background and still avoid detection.  
%
While it is active, the application constantly logs the motion sensors' data including accelerometer, gyroscope and magnetometer readings.
%
The recorded sensor data is stored locally and then later sent to a remote server for processing.

%We also assume that the attacker is able to mark the timestamps when a user begins and ends writing with the Pencil on the screen.
%
%The attacker uses the changes in variance in the magnetometer, accelerometer and gyroscope readings when a user is writing to estimate the beginning and end of the Pencil's interaction with the screen (details described in section~\ref{sec:pencil_orientation_tracking}).
%
In addition, for launching a successful attack, we assume that the attacker is able to obtain or learn a model that captures the human writing behavior.
%
This model's goal is to predict how the Pencil's movement changes over time based on the previous locations of the Pencil.
%
The attacker could train such a model by collecting handwriting data (various letters, numbers, shapes etc.) from a small number of people (up to 3 users is sufficient for the attack to succeed, as shown in the evaluation section).
%
Here, we want to emphasize that these handwriting samples are not collected from the potential attack targets and are solely obtained from the attacker and its accomplices.
%
For training such a model, the attacker uses a computer vision based method (described in section~\ref{sec:map_generation}) for tracking the Pencil's orientation along with logging the Pencil's location and the motion sensors' data.
%
Once trained, the attacker can use it for effectively inferring the free form handwriting of unaware users solely through collecting motion sensor data.
%
Note that the location and orientation information is collected only during training process and at attack time, the attacker does not have access to the location and orientation of the Pencil.




==> miscellaneous/background.tex <==
\section{A First Look}
Observations:

Different letters written at a fixed location on the iPad screen with a fixed orientation for holding the Pencil have different impact on the magnetic readings in all three directions.
%
The same letter written at different locations on the iPad screen with fixed as well as different orientations has different impact on the magnetic measurements.



==> miscellaneous/design_details.tex <==
\section{Design Details}

\subsection{Pencil's Location Tracking}
In our quest for inferring the user's writing from the magnetic data, we begin by exploring the simplest case:
%
Assume that the user always holds the Pencil in a fixed orientation i.e. the 3D orientation of the Pencil does not change, as the user writes on the screen.
%
More specifically, we assume the Pencil is held vertically with altitude of $90^\circ$.
%
In this case, to track how the Pencil moves on the screen, we first determine a mapping between the magnetic readings and the location of the Pencil tip only, since the orientation stays the same.

\subsubsection{2D Magnetic Map}
In order to build the magnetic field map, we have to determine the variation in the magnetic field caused by the Pencil at each location on the iPad screen.
%
The 2D magnetic field map would be a function, $f$, that returns us the magnetic readings corresponding to a given location on the screen i.e.

\begin{equation}
(m_x, m_y, m_z) = f(x, y)
\end{equation}
where $x$ and $y$ are the coordinates of the Pencil tip location and $m_x$, $m_y$ and $m_z$ are the the magnetic reading in $x$, $y$ and $z$ directions.

To build this map, we use a custom drawing application that logs the touch data for the Apple Pencil.
%
iOS's API provides the location of the touch ($x$ and $y$ coordinates of the screen in pixels) of the Pencil.
%
The API scans for a touch at a rate of $120$ times per second.
%
The magnetic data is recorded through a background music player application which can access the magnetometer data.
%
The magnetic data is recorded at a frequency of $50$Hz.
%  
%For a 12.9" iPad Pro, the screen is $155.8mm$ wide and $222.6mm$ in length, with a pixel resolution of ??.
%
Based on iOS API's touch coordinates, we consider the shorter edge of the iPad as $x$ axis and the longer edge as $y$ axis.
%
Instead of tediously finding the magnetic variation for each pixel of the screen, we divide the screen into a gxg grid such that each grid has x pixels.
%
For each grid, we hold the Apple Pencil such that it's tip is touching the center point of the grid, for a few seconds.
%
To keep the Pencil's orientation constant, we ensure that the Pencil is vertical and its rotation does not change.
%
In total, we collect the touch data from the Pencil for $150$ points ($\langle x, y \rangle$ coordinate pairs).
%
The background application is started a few minutes before the Pencil is used to draw the dots in the grids.
%
This allows sensing the ambient magnetic field i.e. magnetic field in the surrounding before there is any impact from the Pencil.
%
Figure ?? shows an example of how the Pencil is held during the map building process.
%
\begin{figure}[h!]
	\centering
	\includegraphics[height=2in, width=2in]{figures/designDetails/2D_vertical_picture.pdf}
	\caption{pencil vertical}
	\label{fig:vertical_pencil}
\end{figure}

After the touch and magnetic data are collected from the described procedure, the touch samples collected for each grid are separated and the average location of the Pencil within each grid is calculated.
%
The timestamps recorded with the magnetic and touch data are used to align the magnetic readings with each of the touch sample. 
%
The average of the ambient magnetic data samples is subtracted from the magnetic readings corresponding to the touch samples to eliminate the magnetic impact of the surroundings.
%
Since the Pencil is held at only the center of each grid, the magnetic field readings at each pixel of the iPad are obtained by interpolation.
%

Figure~\ref{fig:2dmap} shows the interpolated 2D magnetic field map in the $x$, $y$ and $z$ directions. 
%
The axes for the map are measured in millimeters, representing the width and height of the drawable region of the iPad screen.

\begin{figure}[t!]
	\begin{subfigure}{0.32\linewidth}
		\centering
		\includegraphics[width=1.2in]{figures/designDetails/2Dmap_X.pdf}
		\label{fig:2dmap_x}
	\end{subfigure}
	\begin{subfigure}{0.32\linewidth}
		\centering
		\includegraphics[width=1.2in]{figures/designDetails/2Dmap_Y.pdf}
		\label{fig:2dmap_y}
	\end{subfigure}
	\begin{subfigure}{0.32\linewidth}
		\centering
		\includegraphics[width=1.2in]{figures/designDetails/2Dmap_Z.pdf}
		\label{fig:2dmap_z}
	\end{subfigure}
	\caption{2D magnetic map}
	\label{fig:2dmap}
\end{figure}

Once we have build the 2D magnetic map, we ask the question: \textit{how can we track the location of the Pencil using only the magnetic data?}
%
Here we realize that we can benefit from the existing approaches for object tracking in robotics and signal processing.
%
We consider \textit{particle filter}, a popular state estimation algorithm, to track the Pencil's location.

\begin{figure}[t!]
	\begin{subfigure}{0.32\linewidth}
		\centering
		\includegraphics[width=1.1in]{figures/designDetails/2Dpf_A.pdf}
		\label{fig:2dpf_a}
	\end{subfigure}
	\begin{subfigure}{0.32\linewidth}
		\centering
		\includegraphics[width=1.1in]{figures/designDetails/2Dpf_hello.pdf}
		\label{fig:2dpf_hello}
	\end{subfigure}
	\begin{subfigure}{0.32\linewidth}
		\centering
		\includegraphics[width=1.1in]{figures/designDetails/2Dpf_square.pdf}
		\label{fig:2dpf_shape}
	\end{subfigure}
	\caption{2D particle filter}
	\label{fig:2dparticle_filter}
\end{figure}

\subsubsection{2D Particle Filter}
We define the model for the Pencil movement as:
\begin{equation}
s_{t+1} = s_t+ b_t
\label{eq:2dparticle_transition}
\end{equation}
where $s_t$ represents the state vector which is the estimated location of the Pencil tip ($\langle x, y \rangle$ coordinates in millimeter) at time $t$ in our case.
%
$b_t$ is a random perturbation added to the state, with a Gaussian distribution.
% 

The magnetic reading measurement, $q_t$, is represented as:

\begin{equation}
q_t = f(s_t) + e_t 
\label{eq:2dparticle_measurement}
\end{equation}
where $e_t$ is the noise in the sensor measurement with a zero-mean Gaussian distribution $p_{e_t}$.
%
$f$ is the 2D map function generated from the process described in the last section.
%We define of the location of the Pencil tip ($\langle x, y \rangle$ coordinates of the screen in millimeter) at time $t$ as the state vector $s_t$.
%
We begin by generating $s_0^i \sim p_{s0}$ where $s_0$ represents the initial state of the particles and $i = 1 . . . N$.
%
%
These particles are initially uniformly spread all over the screen.
%
Weights are assigned to each particle at each time step with the likelihood function:
\begin{equation}
%w_t^i = w_{t-1}^i p(u_t|s_t^i) =  w_{t-1}^i p_{e_t}(dist(u_t, f(s_t^i)))
w_t^i = \exp(\frac{(q_t - m_t)^2}{\sigma})
\label{eq:2dparticle_weight}
\end{equation}
Here $m_t$ is the magnetic readings obtained from the magnetometer at time $t$. 
%
We use Euclidean distance to measure the difference between the estimated and measured magnetic readings.
%
The weights calculated from the likelihood function are normalized such that the sum of weights of all particles is equal to $1$.
%
These weights basically determine how likely the Pencil tip is to be at the location depicted by a particle at time $t$.
%
Therefore, particles with higher weights should be given a higher priority than the lower weights one.
%
At each time step, the particles are resampled based on these weights such that the particles whose weights are above a threshold, $\tau$ are replicated to replace the particles whose weights are below $\tau$.
%
The movement of the particles is governed by equation~\ref{eq:2dparticle_transition}.
%\begin{equation}
%s_{t+1} = s_t + e_t
%\end{equation}
%$e_t$ is the noise in the sensor measurement with a zero-mean Gaussian distribution $p_{e_t}$.
%
The particle with the maximum weighted average is chosen as the location of the Pencil tip at each time stamp.
%

Figure~\ref{fig:2dparticle_filter} shows the results of this naive implementation of particle filter when used to track a letter (\textit{'A'} - Figure~\ref{fig:2dpf_a}), a word(\textit{'hello'} - Figure~\ref{fig:2dpf_hello}) and a shape (a square - Figure~\ref{fig:2dpf_shape}).
%
The figure shows the ground truth and the tracking results from 2D particle filter.
% 
Here, even though we do not use any trend information in the particle transition function, we are able to track the Pencil movement pretty well.
%
Thus, the usage of particle shows promise for tracking what the user is writing.

\subsection{Pencil's Orientation and Location Tracking}
Now that we have solved the simple case of inferring what is written on the screen with a fixed orientation of the Pencil, we proceed to the more general and realistic case:
Assume that the user can write with their natural free-form writing style.
%
This means that we have to relax the constraints on the Pencil's orientation during writing.
%
In this case, the magnetic field map needed for tracking the Pencil movement is a function, $f$, mapping the location $\langle x, y \rangle$ of the Pencil tip and its 3D orientation to the magnetic readings in $x$, $y$ and $z$ directions i.e.
\begin{equation}
(m_x, m_y, m_z) = f(x, y, orientation)
\label{eq:5dmap}
\end{equation}
%

For building this magnetic map, we first want to introduce the coordinates systems for the iPad screen and the Pencil and clarify the notion of the Pencil's orientation.

\subsubsection{iPad Screen and Pencil Coordinate Systems}

\begin{figure}[h!]
	\centering
	\includegraphics[height=1.5in, width=2in]{figures/designDetails/coordinate_systems.pdf}
	\caption{coordinate systems}
	\label{fig:coordinate_systems}
\end{figure}

\begin{figure}[h!]
	\centering
	\includegraphics[height=2.5in, width=2in]{figures/designDetails/camera_setup.pdf}
	\caption{camera setup}
	\label{fig:camera_setup}
\end{figure}

Figure~\ref{fig:coordinate_systems} shows the coordinate systems for the iPad screen, $C_s$.
%
The top-left corner of the iPad screen is the origin for $C_s$.
%
The location of the Pencil tip reported by the iOS touch API is also in the screen coordinate system.
%
As shown in the figure, the $Z$ axis of $C_s$ points downwards based on the right hand rule.
%
Figure~\ref{fig:coordinate_systems} also shows the $X$, $Y$ and $Z$ axes of the Pencil local to its own coordinate system, $C_p$.
% 
The $Z$ axis of the Pencil runs vertically through the Pencil body.
%

\subsubsection{Pencil's 3D orientation}
%TODO is this correct?
We define the orientation of the Pencil as its axes expressed as vectors in the screen coordinate system denoted as $X_{ps}$, $Y_{ps}$ and $Z_{ps}$.
%
To be able to determine the orientation of the Pencil as it moves, we need to find how the Pencil's axes rotate in $C_s$. 
%The orientation of the Pencil can be defined by any rotation around its axes.
%
iOS touch API for Apple Pencil provides the altitude and azimuth angles between the Pencil and the iPad screen.
%
%The altitude angle is the angle between the $Z$ axis and the $XY$ plane of the Pencil while the azimuth angle is the angle between the projection of Pencil's $Z$ axis onto the $XY$ plane and its $X$ axis.
%
These two angles do not provide any information about the Pencil's rotation about its $Z$ axis.
%
Without considering this rotation, we cannot fully describe the Pencil orientation and hence estimate the impact of the Pencil on the magnetic readings accurately.
%

Therefore, we consider using computer vision techniques for determining the 3D orientation of the Pencil.
%
%TODO find reference
Suppose we can record the movement of the Pencil with a camera during map building process, we can use 3D pose estimation to determine the 3D orientation of the Pencil using images captured by the camera.
%
3D pose estimation operates by finding the 3D rotation and translation of an object from an image, if an approximate 3D model of the object and the corresponding points in the 2D image are known.
%
To this end, we record the Pencil movement with a camera placed at a distance above the iPad and looking down upon the screen.
%
Figure~\ref{fig:camera_setup} shows the setup.
%
For pose estimation to work, the camera needs to be calibrated first.
%
We calibrate the camera by showing an image of a checkerboard pattern (similar to the pattern shown in Figure~\ref{fig:coordinate_systems}) on the iPad screen.
%
The iPad is moved to capture several images with different distances and orientations of this pattern with respect to the fixed camera.
%
The images are given as input to camera calibration algorithm to find the extrinsic and intrinsic parameters of the camera.
%
These parameters are then used to find the location and orientation of the camera in $C_s$.
%

Once the camera is calibrated, we attach a checkerboard to the Pencil end to estimate its pose and in turn the Pencil's 3D orientation.
%
Figure~\ref{fig:coordinate_systems} also shows the 3D coordinate system of the checkerboard, $C_b$.
%
We define the center point of the checkerboard as the origin of $C_b$ and measure the coordinates of the square corners in $C_b$ to approximate the checkerboard's 3D model.
%
Checkerboard detection is applied to the images recorded by the camera as the Pencil moves on the screen to find the corresponding points in the images.
%
%TODO find reference
Given the 2D points from the image and the 3D points defined in checkerboard coordinate system, we use PnP algorithm to estimate the 3D coordinates of the camera center and its 3D rotation in $C_b$ space.
%
This camera center and orientation is then used to transform the checkerboard axes and its origin (center) into the screen space, $C_s$.
%
Because of the noise in camera calibration and pose estimation steps, the center coordinates and the orientation are noisy.
%
To remove this noise, we convert the 3D orientation of the checkerboard into quaternions and apply Kalman filtering and smoothing to the quaternions obtained over time.  
% 
Since the checkerboard's origin is attached to the Pencil end, the 3D axes of the checkerboard in $C_s$ obtained after smoothing are indeed the axes of the Pencil in $C_s$ as well.
%
Therefore, by tracking the axes of the checkerboard, we can track the orientation of the Pencil as it moves on the screen.

\subsubsection{3D Map Generation}
%
Now that we can track the orientation of the Pencil, we get back to building the magnetic map for the five parameters of Pencil's position i.e.
%
\begin{equation}
(m_x, m_y, m_z) = f(x, y, X_{ps}, Y_{ps}, Z_{ps})
\end{equation}
%
For this case, even if we use grids on the screen, we need to move the Pencil in all possible orientations within each grid to get the magnetic impact for each orientation.
%
Determining the magnetic readings corresponding to every orientation through war driving requires a huge amount of human effort.
%
Hence, we focus on opportunities to reduce the war driving space for building the magnetic field map.

\begin{figure}[h!]
	\centering
	\includegraphics[height=2in, width=2in]{figures/designDetails/pencil_states.pdf}
	\caption{different pencil orientations}
	\label{fig:pencil_states}
\end{figure}

%
So far we have considered building the magnetic map from the iPad's perspective i.e. the Pencil's position and magnetic readings are all considered to be in the screen coordinate system, $C_s$.
%
Another way to look at this problem is to build the map from the Pencil's perspective.
%
Recording the magnetic impact of the Pencil movement on the screen is essentially the same as keeping the Pencil stationary and moving the magnetometer around it.
%
In other words, for any position of the Pencil in $C_s$, we can find the corresponding magnetometer position in $C_p$.
%
%In other words, if we consider Pencil's coordinate system, $C_p$, where the Pencil tip's coordinates are always $[0, 0, 0]$, as the Pencil moves on the screen, the magnetometer moves and rotates in $C_p$.
%
Given that we know the location of the magnetometer, $M_{loc}$, in $C_s$, if the Pencil tip is at location, $T_{loc}$, the location of the magnetometer in $C_p$, $M_{loc^\prime}$ can be represented by 
%
\begin{equation}
M_{loc}^\prime = P_{s}*(M_{loc}-T_{loc})
\label{eq:mloc}
\end{equation}
where $P_s$ is the tuple $(X_{ps}, Y_{ps}, Z_{ps})$ representing Pencil's axes in screen space.

Similarly, we can also transform the magnetic readings in $C_s$, $m_r$ to magnetic readings in $C_p$, $m_r^\prime$ by
\begin{equation}
m_{r}^\prime = P_{s}*m_r
\label{eq:mr}
\end{equation}


\begin{figure*}[t!]
	\centering
	\begin{subfigure}{0.32\linewidth}
		\centering
		\includegraphics[width=2.3in]{figures/designDetails/pencilMap_before_minus5.pdf}
		\label{fig:pencilMap_before_minus5}
	\end{subfigure}
	\begin{subfigure}{0.32\linewidth}
		\centering
		\includegraphics[width=2.3in]{figures/designDetails/pencilMap_before_0.pdf}
		\label{fig:pencilMap_before_0}
	\end{subfigure}
	\begin{subfigure}{0.32\linewidth}
		\centering
		\includegraphics[width=2.3in]{figures/designDetails/pencilMap_before_5.pdf}
		\label{fig:pencilMap_before_5}
	\end{subfigure}
	\begin{subfigure}{0.32\linewidth}
		\centering	\includegraphics[width=2.3in]{figures/designDetails/pencilMap_after_minus5.pdf}
		\label{fig:pencilMap_after_minus5}
	\end{subfigure}
	\begin{subfigure}{0.32\linewidth}
		\centering	\includegraphics[width=2.3in]{figures/designDetails/pencilMap_after_0.pdf}
		\label{fig:pencilMap_after_0}
	\end{subfigure}
	\begin{subfigure}{0.32\linewidth}
		\centering	\includegraphics[width=2.3in]{figures/designDetails/pencilMap_after_5.pdf}
		\label{fig:pencilMap_after_5}
	\end{subfigure}
	\caption{TBD}
	\label{fig:pencilMap}
\end{figure*}

This means that for any two points on the screen which are at the same distance from $M_{loc}$, their corresponding $M_{loc}^\prime$ will be the same in Pencil's coordinate space. 
%
Figure~\ref{fig:pencil_states} shows an example of two Pencil positions which are different in $C_s$, however from Pencil's perspective, the magnetometer will be at the same location in $C_p$ for these two positions.

The benefit of building a map around the Pencil is that it reduces the search space for war driving from 5D to 3D space, since now we only need to cover all the possible 3D locations of the magnetometer in $C_p$.
%
Secondly, $M_{loc}^\prime$ can be the same for more than one Pencil position in $C_s$.
%
Therefore, instead of collecting only one sample for each Pencil location and orientation, we can collect multiple samples for a position in $C_p$ when we move the Pencil at different locations on the screen. 

Considering the benefits mentioned above, we decide to build the magnetic map around the Pencil to capture its magnetic impact with different locations and orientation.
%
For this purpose, we use our setup shown in Figure~\ref{fig:camera_setup} to track the orientation of the Pencil while randomly drawing on the screen.
%
In this random drawing, we try to rotate and move the Pencil such that we can cover the entire screen and maximum possible orientations.
%
This random drawing approach is faster than using a grid based approach and lets us collect multiple sample points for a given Pencil position.
%
Similar to the procedure for building 2D magnetic map, we collect the magnetic data in the background.
%
Once we finish, we have the touch data from the iOS API, the orientation data from the camera and the magnetic data from the magnetometer.
%
The magnetic impact of ambiance is removed from the magnetic readings.
%
For each touch sample, we transform the $M_loc$ and sample's corresponding $m_r$ to $C_p$ using equation~\ref{eq:mloc} and \ref{eq:mr} respectively.
%
These transformed magnetic readings in $C_p$ are finally quantized into $5x5 mm$ grids based on the 3D location of the $M_{loc}$ corresponding to the reading.
%
The average of all the magnetic data samples is computed for each grid.
% 
Figure~\ref{fig:pencilMap} shows the $XY$ plane of this 3D map built around the Pencil for $z = -5$, $z = 0$ and $z = 5$. 

\subsubsection{3D Map Reconstruction}
As shown in Figure~\ref{fig:pencilMap}, some of the grids in the 3D map do not have any samples from the data collected for map generation.
%
To be able to use the 3D map for tracking the Pencil movement for free-form handwriting, we need the map to be complete i.e. we need to account for the missing data.
%
%In order to be able to use the 3D map for tracking, we need to account for the missing magnetic data and deal with the noise in our readings.
%
One may argue that why not simply use interpolation to get the missing data.
%
Although we have a large number of samples in the grids corresponding to the more common orientations of the Pencil, the magnetic readings are impacted by the sensor noise.
%
If this noisy data is directly used for interpolation, the resulting 3D map will not be accurate.
%
In addition, unlike 2D magnetic map, a linear interpolation method cannot be used to determine the magnetic field of the Pencil.
%
Consequently, we need a mechanism to reduce the noise in the collected magnetic data and generate the missing data for the map while considering the properties of magnetic fields in mind.
%

Keeping our requirements for the 3D map in mind, we found a reconstruction algorithm for the magnetic field. 
%
This algorithm consider that the fact that the divergence of the magnetic field should be zero.
%
It operates by minimizing the function:

\begin{equation}
J(g;f) = \sum_{m}|Ag(m)-f[m]|^{2} + \lambda_{c}||curl g||_1 + \lambda_d||div g||_1
\end{equation} 
where $g$ is the reconstructed map and $f$ is the original magnetic map.
%
$A$ is an operator which only selects grids containing at least one datum.
%
$\lambda_c$, $\lambda_d$ are regularization parameters.
%

According to the Maxwell's equations bounding the magnetic field, the regularization parameter, $\lambda_{c}$ should be $0$ while $\lambda_d$ should be really large.
%
%TODO: add reference
However, considering the noise in the magnetic readings, we choose $\lambda_c= 0.3$ and  $\lambda_d = 1.5$ to reconstruct the magnetic map based on the best parameter selection procedure described in ?. 
%
These regularization parameters ensure that the divergence and curl of the magnetic field are not impacted by the noise in the data and are minimized.
%
The resulting 3D magnetic map from this approach is continuous with reduced noise.
%
Figure~\ref{fig:pencilMap} shows the $XY$ plane of this 3D map for $z = -5$, $z = 0$ and $z = 5$ after reconstruction. 

==> miscellaneous/introduction_old.tex <==
\section{Introduction}
% no \IEEEPARstart
Modern day smart devices come embedded with a variety of sensors enabling a vast range of applications in activity recognition, context awareness, mobile health, productivity etc.
%
Despite their invaluable benefits, these sensors can leak information about user's activity.
%
Leakage of users' personal information, revealing their habits, behaviors, and preferences, through sensor data has been a major security concern for a many years.
%
Keeping user privacy in mind, mobile operating systems, like Android and iOS, require users' permission for applications to access sensitive data from sensors like GPS, cameras, and microphones.
%
However, some other sensors like magnetometer, accelerometer and gyroscope can be accessed by applications even without user permission.
%
At a time when smart devices are an essential part of our everyday lives, access to these sensors' data has opened doors to a multitude of side channel attacks.
%

Several prior works have unveiled security vulnerabilities and attacks resultant of applications having open access to motion sensors' data.
%
%One class of such attacks targeted on tracking users' location by making inferences from the motion sensors' data \cite{wang2015mole} \cite{}.
%%
One major category of these attacks focuses on inferring patterns in user activity and behavior from the motion data.
%
These include inferring information about users' touch actions and keystroke detection~\cite{wang2015mole, MehrnezhadTSH16, Maiti2016}, guessing users' passwords and PIN codes ~\cite{owusu2012accessory,MehrnezhadTSH16} and application and webpage fingerprinting~\cite{deepMag, matyunin2019magneticspy}.
%
Although extensive research has been done in this area, each of these works targets specific smart devices and/or platforms. 
%
With frequent software updates and new devices appearing in the market regularly, new security threats arise everyday.
%
\begin{figure}%
%	\centering
	\begin{subfigure}{0.40\linewidth}
		\centering
		\includegraphics[height=2.0in, width=2.0in]{figures/introduction/fig1_img_new.pdf}
		\caption{}
		\label{fig:screen_basic}
	\end{subfigure}	
	\begin{subfigure}{0.58\linewidth}
		\centering
		\includegraphics[height=2.0in, width=3.0in]{figures/introduction/fig1_mag_new.pdf}
		\caption{}
		\label{fig:basic_pattern3d}		
	\end{subfigure}
	\caption{Example of magnetometer readings when a user writes on the iPad using Apple Pencil.}
	\label{fig:basic_word}
\end{figure}

With an ever increasing popularity of tablet devices in the market, many manufacturers have started supporting stylus pencils with their tablets to improve the user experience.
%
In this paper, we direct our attention to the recently launched Apple Pencil (2nd generation) supported with the popular Apple iPad Pro. 
%
Apple Pencil is the Apple's stylus pen which can be used for writing, drawing and making selections on the iPad screen.
% 
To improve its usability and convenience, unlike the 1st generation, the new version of the Pencil pairs wirelessly with the iPad for charging.
%
In order to do so, the Pencil body has magnets embedded in it which allow the flat edge on one side of the Pencil to attach to side of the iPad body magnetically.
%
With the presence of these magnets, the Pencil's body can possibly have an impact on magnetic readings sensed by the iPad when a user is interacting with the screen.
%
To verify this, we record the magnetometer data while a user writes the character `a' on the iPad using the Apple Pencil (shown in Figure~\ref{fig:screen_basic}).
%
%The magnetic data is collected in background through a third party application running an audio player service.
%
%We ensure the audio player plays an inaudible sound file to avoid detection.
%
Figure~\ref{fig:basic_pattern3d} shows the corresponding magnetic readings in X, Y and Z directions recorded by the magnetometer.
%
As shown in the figure, when the Pencil interacts with the screen, there is a visible change in the magnetic readings.
%
While this new feature of the Pencil improves user's experience, the changes in the Pencil's body have opened the door to a potential privacy leakage.
%

%
Therefore, we ask the question: \textit{Can we infer what a user is writing on the iPad screen with the Apple Pencil, given access to only the motion sensors' data?} 
%
iOS does not allow third party applications running in the background to access the touch information (position of the Pencil tip) when a user is writing for example.
%
However because of the loop hole in iOS's access control, any background application can easily log the magnetic field data, accelerometer data and gyroscope data without needing to request any permissions.
%

\begin{figure}[ht!]%
	\begin{subfigure}{0.45\linewidth}
		\centering
		\includegraphics[height=2in, width=1.5in]{figures/introduction/abc.pdf}
		\caption{}
		\label{fig:screen_differentletters}
	\end{subfigure}	
	\begin{subfigure}{0.45\linewidth}
		\begin{subfigure}{1\linewidth}
			\centering
			\includegraphics[height=0.66in, width=1.8in]{figures/introduction/abc_magX.pdf}
		\end{subfigure}
		%\label{fig:basic_pattern3d}
		\begin{subfigure}{1\linewidth}
			\centering
			\includegraphics[height=0.66in, width=1.8in]{figures/introduction/abc_magY.pdf}
			%\label{fig:basic_pattern3d}
		\end{subfigure}		
		\begin{subfigure}{1\linewidth}
			\centering
			\includegraphics[height=0.66in, width=1.8in]{figures/introduction/abc_magZ.pdf}
			%\label{fig:basic_pattern3d}
		\end{subfigure}
		\caption{}
		\label{fig:mag_differentletters}
	\end{subfigure}
	\caption{The magnetometer readings change when a user writes different characters on the screen.}
	\label{fig:different_letters}
\end{figure}

As observed in Figure~\ref{fig:basic_word}, determining when a user is using the Pencil on the screen from the magnetic data is trivial.
%
%However, figuring out any meaningful information from the magnetic data involves some serious challenges. 
%
In our preliminary experiments, we observed that the impact of the Pencil on the magnetic readings changes with what the user is writing on the screen.
%
Figure~\ref{fig:different_letters} shows one such example.
%
We wrote the letters `a', `b' and `c' on the iPad screen and recorded the magnetometer data (shown in Figure~\ref{fig:screen_differentletters}).
%
Figure~\ref{fig:mag_differentletters} shows the magnetometer readings in the three axes.
%
We can see that the fluctuations in the magnetometer readings are different for each of the three characters.
%
One intuitive approach is to train a learning model that takes into account the similarity between the magnetic data over time for a given set of alphabet to determine any useful patterns like letters, numbers or shapes drawn on the screen.
%
Although intuitive, this approach would only work if the magnetic impact of the Apple Pencil is consistent when the Pencil is held at different locations or with different orientations on the iPad screen for a given letter, number or shape.
%



\begin{figure}[t!]%
	\begin{subfigure}{0.45\linewidth}
		\centering
		\includegraphics[height=2in, width=1.5in]{figures/introduction/four_as.pdf}
		\caption{}
		\label{fig:screen_different_locations_orientations}
	\end{subfigure}	
	\begin{subfigure}{0.45\linewidth}
		\begin{subfigure}{1\linewidth}
			\centering
			\includegraphics[height=0.66in, width=1.8in]{figures/introduction/four_as_magX.pdf}
		\end{subfigure}
		%\label{fig:basic_pattern3d}
		\begin{subfigure}{1\linewidth}
			\centering
			\includegraphics[height=0.66in, width=1.8in]{figures/introduction/four_as_magY.pdf}
			%\label{fig:basic_pattern3d}
		\end{subfigure}
		
		\begin{subfigure}{1\linewidth}
			\centering
			\includegraphics[height=0.66in, width=1.8in]{figures/introduction/four_as_magZ.pdf}
			%\label{fig:basic_pattern3d}
		\end{subfigure}
		\caption{}
	\end{subfigure}
	\caption{The magnetometer readings change when a user writes the same character on the screen.}
	\label{fig:different_locations_orientations}
\end{figure}

%\begin{figure}%
%	\begin{subfigure}{0.45\linewidth}
%		\centering
%		\includegraphics[height=2in, width=1.5in]{figures/introduction/four_as.pdf}
%		%\label{fig:pattern_basic}
%	\end{subfigure}	
%	\begin{subfigure}{0.45\linewidth}
%		\centering
%		\includegraphics[height=2in, width=2in]{figures/introduction/four_as_mag.pdf}
%		%\label{fig:basic_pattern3d}
%	\end{subfigure}
%	\caption{different a's}
%	\label{fig:different_locations}
%\end{figure}
To determine whether this is the case for Apple Pencil and iPad, we wrote the character `a' with the Pencil at different locations and different orientations on the iPad screen.
Figure~\ref{fig:screen_different_locations_orientations} shows two `a's written in different locations - $a_1$ and $a_3$, as well as two `a's in the same location but the Pencil was rolled $180^\circ$ - $a_3$ and $a_4$. Although the traces of characters visually look the same,  magnetometer readings vary significantly. 

%
%Figure~\ref{fig:screen_different_locations_orientations} shows two `a's written in different locations - $a_1$ and $a_3$.
%
%The range of the axis is given in millimeters corresponding to the iPad screen.
%
%Although the two characters visually look the same, their magnetic trends are very different.
%
%Similarly, given the nature of human writing behavior, even when writing at the same location, a user might not hold the Pencil in a particular orientation always.
%
%Figure~\ref{fig:screen_different_locations_orientations} shows two `a' in the same location but the Pencil is rolled $180^\circ$ - $a_3$ and $a_4$. % such that the flat edge of the Pencil is facing a different direction than that for the previous 'a'.
%
%Again, the two `a's look similar visually however their magnetometer readings vary significantly from each other.
%
%Furthermore, patterns found in the writing behavior would hugely vary across different people since people have different writing styles.
%

Based on these observations, in order to launch an attack aiming at inferring information about user's writing,  we design a tracking algorithm to track the Pencil tip movement using magnetic field data.
%
Building such an algorithm requires finding the mapping between a given magnetic reading and the Pencil tip's location and its orientation with respect to the screen.
%
%For most note taking and drawing applications, Pencil can be used anywhere on the iPad screen and can be held in any orientation. 
%
%This means that the range for Pencil location is basically the width and height of the iPad screen.
%
%The orientation of the Pencil is mainly determined by the altitude and azimuth of the Pencil's body with respect to the screen.
%
%In addition, the Pencil can be held with it's flat edge being rotated from $0$ to $360^\circ$.
%
%All in all, the mapping between the magnetic trend and the Pencil location and orientation would be determined by the $5$ parameters of the Pencil.
%
A common method for finding such mappings is wardriving.
%
However, in our case, the space for this mapping is $5$ dimensional since we want to track the 2D location of the Pencil on the screen while keeping record of its 3D orientation. %where each dimension has a huge possible range.
%
Wardriving for all possible locations and orientations of the Pencil on the iPad requires a huge amount of human effort.
%
We minimized this effort by building the magnetic field map around the Pencil instead of determining the magnetic field for the screen.
%
With this mapping, we design a particle filter~\cite{particleFilter} which tracks the locations of the Pencil on the iPad screen solely based on the data collected from the motion sensors.
%
We leverage the human writing behavior to guide the particles' initialization and transition in particle filter to improve the tracking accuracy.
%HF - needs fixing
%Considering the aforementioned challenges, this paper presents, ?, which aims at determining what a user is writing or drawing with the Apple Pencil with access to only the magnetometer's data.
%%
%We build a $5$ dimensional particle filter which considers all the possible locations and orientations of the Pencil on the iPad screen.
%%
%Given the magnetic data, the particle filter tracks the movement of the Pencil.
%%
%To guide the movement of the particles, we build a magnetic map serving as bridge between the magnetic data and the Pencil position.
%%
%We reduce the search space for wardriving to build this map by assuming the Pencil's position is fixed and determine the position of the magnetometer with respect to the Pencil's tip as it moves on the screen.
%%
%This way, we only need to track the 3D orientation of the magnetometer with respect to the Pencil, hence greatly reducing the search space.
%%

We implemented our system, \sys (\textbf{S}ide-channel attack on \textbf{S}tylus pencil through \textbf{S}ensors), on Apple 11" iPad Pro running iOS 12.0.
%
To evaluate \sys, we conducted experiments with $10$ subjects, where the subjects wrote different letters, shapes and numbers at different locations of the screen.
%
The attacker was able to correctly guess $93.9\%$, $96\%$ and $97.9\%$ of the letters, numbers and shapes respectively.
%
Our system also tracked different English words with an accuracy of $91.67\%$.
%Our system can track the letters, numbers and shapes with an average accuracy of ??.

The main contributions of this paper can be summarized as:
\begin{itemize}
	\item Unveiling the privacy leakage through motion sensor data from modern tablets due to the introduction of stylus pencils with embedded magnets. We build a system which can track user's writing by generating a magnetic map of the Pencil and designing a particle filter to track its movement.
	\item Implementing our system on iPad Pro with Apple Pencil and demonstrate good accuracy for inferring letters, numbers and shapes across $10$ subjects.
\end{itemize}

\vspace{0.1in}


==> response.tex <==
\section*{Letter to Reviewers}
Dear Reviewers,

We would like to thank you for your insightful reviews and valuable comments and suggestions.
%
We have addressed all the major revision requirements and comments from reviewers in our paper.
%
The following is a summary of our changes to address the requirements for major revision (Section A) as well as the comments in individual reviews (Section B). 
%
For your convenience, we will repeat some of the new contents we added to the paper in this letter as well - please pardon the redundancy.
%

In the main text of this PDF (above this letter), you will find tags such as \textbf{[MRx]} and \textbf{[Cx]} along with highlighted text to point to the added/revised contents of the paper which correspond to the specific major revision item or individual comments from the reviewers respectively.

Additionally, for your review convenience, we have attached a PDF diff version showing all our revisions and changes since the last submission, \emph{after} this letter.

Thank you.

\vspace{1mm}\noindent Sincerely,

\noindent Authors of Submission \# $5009$

\setcounter{section}{0}
\section{Response to Major Revision Requirements}

We thank the $1$AE for summarizing the reviewers' comments and listing requirements for the major revision. Following is the summary of our changes in response to these requirements.

\vspace{2mm}\noindent\textbf{MR1: The motivations of the paper is weak and is not sufficient in convincing the need for the use of the proposed system (R2, R3).
}

We address this comment in the introduction (Section~\ref{sec:introduction}) and threat model (Section~\ref{sec:threat_model}) of the paper.
%
We highlight that users often use Apple Pencil to enter text in any of the text fields in various applications~\cite{pencil20scribble}.
%
This means that an adversary capable of inferring a user's handwriting through the motion sensors' data can infer its private information such as text messages, signatures, passwords, and notes.
%
%%

\vspace{2mm}\noindent\textbf{MR2: The revision should reflect how the system will perform in real use case scenarios (R2 R3). How will the system perform with data never seen before? How will the training take place with a small amount of data?
}

The only component of \sys{} that needs user data for training is the writing behavior model.
%
We explained in the threat model (Section ~\ref{sec:threat_model}) that this model can be trained by collecting handwriting data such as letters, numbers, shapes, etc., from a small number of users.
%
To support this claim, we collected data from $3$ users to train the writing behavior model in our evaluation.
%
The $3$ users were not included in the $10$ subjects in our evaluation set.
%
Therefore, all of our evaluation results are based on unseen data.
%
\sys{}'s high detection accuracy shows that a small amount of training data is sufficient for the writing behavior model to precisely guide the particle filter.
%%

\vspace{2mm}\noindent\textbf{MR3: More realistic evaluations are needed (R2, R3, R4). The evaluations should additionally consider practical interference factors (R2, R4), offer end-to-end evaluations (R3), and in-the-wild evaluations (R3, R4).}

We added three new evaluations in Section ~\ref{sec:evaluation} to demonstrate the practicality of our system, (1) interference factors, (2) end-to-end evaluations, and (3) in the wild evaluations, detailed below.
%%

\vspace{1mm}\noindent\textbf{(1) Interference factors:} We conducted additional experiments to evaluate the impact of practical interference.
%
We observed that regular objects such as clothes and books in the environment do not impact the magnetic readings sensed by the iPad's magnetometer.
%
We also recorded the impact of opening or closing the door and people walking in the surroundings (common activities) while a user is writing on the iPad.
%
\sys{}'s performance is not significantly affected by such changes in the environment.
%
Additionally, we conducted experiments for two scenarios to evaluate \sys{}'s performance under interference when (1) a user wears a watch with a magnetic bracelet on their wrist and (2) a smart folio case for the iPad is used. In these scenarios, $3$ subjects were asked to write letters, numbers, and shapes on the iPad.
%
Table~\ref{table:environment2} summarizes the results of our experiments.
%
In scenario $1$, despite having the magnetic bracelet very close to the iPad, the Pencil's magnetic impact is still stronger, allowing \sys{} to track the Pencil movement.
%
For the smart folio case, we observe that its magnetic impact is consistent over time, and \sys{} is able to separate the impact of the Pencil as it moves on the screen. 

\vspace{1mm}\noindent\textbf{(2) End-to-end evaluations:} We added an end-to-end attack with \sys{} by considering a real-world scenario where the victim uses the Pencil to write a text message in a chatting application.
%
We invited $3$ volunteers to write $10$ different valid English sentences used in text message conversations (without punctuation and emojis).
%
We used stroke detection to separate the magnetic readings for different words within each sentence and fed them to our particle filter.
%
The tracking results were then shown to a volunteer pretending to be an attacker (not included in the $3$ test subjects).
%
The attacker correctly guessed $66.67\%$ of all the words in the first three guesses.
%
We observed that due to the short duration between writing different words in a sentence, the tracking results for some of the strokes are noisy, making it difficult to accurately guess some words.
%
However, once the tracking results of all the words in a given sentence were shown together as a sentence, the attacker could guess $80\%$ of the sentences correctly by interpreting the semantic relations between words.
%
%reviewing below, will finish soon.
%%

\begin{table}[t!]
\centering
\begin{tabular}{ |c | c| c| c|}
\hline
 Scenario & Letters ($\%$) & Numbers ($\%$) & Shapes ($\%$) \\ 
\hline
 Door opening and closing & 93.37 & 95.55 & 96.67 \\  
 People walking around in the room & 93.80 & 96.58 & 97.86 \\
 Watch with metallic bracelet & 91.88 & 95.55 & 96.67 \\
 Smart folio iPad case & 91.67 & 94.44 & 96.67 \\
\hline
\end{tabular}
\caption{\sys{}'s detection accuracy in different environmental settings.}
\label{table:environment2}
\end{table}


\vspace{1mm}\noindent\textbf{(3) In the wild evaluations:}
We added experiments in our evaluation in Section~\ref{sec:evaluation} while users are writing with a variety of iPad positions.
%
In addition to the simple case where iPad is placed on a table, we evaluated the following four scenarios: (1) iPad is held in hand while sitting, (2) iPad is held in hand while standing, (3) iPad is held in hand while laying down, and (4) iPad is held in hand while walking.
%
We added the results of the experiments conducted in each of the four scenarios in Figure~\ref{fig:performance_hand2}.
%
We note that although holding the iPad in hand causes tiny fluctuations in the magnetic readings, these changes are much smaller than the fluctuations caused by the Pencil.
%
Therefore, \sys{} can track the Pencil with an accuracy higher than $90\%$ in the first three scenarios.
%
In the case where the user is walking, \sys{}'s accuracy deteriorates ($66.2\%$, $77.8\%$ and $87.8\%$ for letters, numbers and shapes respectively) since the ambient magnetic field changes frequently, making it difficult for our system to separate it from the Pencil's magnetic impact.
%
%%

\begin{figure}[t!]
	\centering
	\begin{subfigure}{0.24\linewidth}
		\centering
		\includegraphics[height=1in]{figures/evaluation/performance_hand_sitting.pdf}
		\caption{}
		\label{fig:performance_hand_sitting2}
	\end{subfigure}
	\begin{subfigure}{0.24\linewidth}
		\centering
		\includegraphics[height=1in]{figures/evaluation/performance_hand_standing.pdf}
		\caption{}
		\label{fig:performance_hand_standing2}
	\end{subfigure}
	\begin{subfigure}{0.24\linewidth}
		\centering
		\includegraphics[height=1in]{figures/evaluation/performance_hand_laying.pdf}
		\caption{}
		\label{fig:performance_hand_laying2}
	\end{subfigure}
	\begin{subfigure}{0.24\linewidth}
		\centering
		\includegraphics[height=1in]{figures/evaluation/performance_hand_walking.pdf}
		\caption{}
		\label{fig:performance_hand_walking2}
	\end{subfigure}
	\caption{Accuracy of the correctly guessed letters, numbers and shapes in 1, 2 and 3 guesses when the user is holding the iPad in hand (a) while sitting, (b) while standing, (c) while laying down, and (d) while walking.}
	\label{fig:performance_hand2}
\end{figure}

\vspace{2mm}\noindent\textbf{MR4: While the authors discuss the use of deep models in the discussions, given the interest in the field, it would be meaningful to present performance-level comparisons with deep learning models designed for the same purpose (R2).}

We compared the performance of \sys{} with different machine learning techniques in Section~\ref{sec:evaluation}. 
%
We implemented three different state-of-the-art models to infer the users' handwriting from the magnetic readings and evaluated it on the data collected from the $10$ subjects in our user study. The models are built using (1) k-nearest neighbors (k-NN) regression model, (2) Long Short Term Memory networks (LSTM) model for classification, and (3) an ensemble of LSTM models for classification trained for different locations of the iPad screen. 
%
%\berkay{Why these algorithms?  You can copy and paste text from evaluation}.
We selected these algorithms as they capture the order dependence in our dataset and consider the nearest neighbors or previous states of the pencil while guiding us about the pencil location over time (we have added details of these models in the Appendix.)
%
With the same dataset used in the particle filter algorithm, these models were unable to precisely capture the relationship between the changes in the Pencil's location and orientation and the sensed magnetic readings.
%
As a result, the accuracy of these models is much lower compared to \sys{}. 
%
More specifically, the k-NN model allowed the attacker to guess only $11.54\%$, $18.67\%$, and $3\%$ of the letters, numbers and shapes, respectively.
%
Similarly, the LSTM model achieved an accuracy of $7.69\%$, $10\%$, and $21.67\%$ for letters, numbers, and shapes, respectively.
%
The ensemble of LSTM models for different iPad screen locations could only improve the accuracy to $11.54\%$, $16.67\%$, and $29.67\%$ for letters, numbers, and shapes, respectively.
%
In contrast, \sys{} was able to identify $93.9\%$, $96\%$ and $97.9\%$ of the letters, numbers, shapes, correctly by using particle filter on the same dataset.
%
\sys{}'s multi-dimensional particle filter considers both the Pencil's location and orientation in the previous states when predicting the current Pencil location and uses the particles' history to track the Pencil movement precisely, producing more accurate results.
%%

\vspace{2mm}\noindent\textbf{MR5: An improved threat model is needed in the manuscript (R3, R4). As a reader, it is hard to link the threat model with the proposed approach and the findings from the evaluations.}

We revised our threat model (Section~\ref{sec:threat_model}) to clarify our assumptions in light of the recent iOS updates limiting motion sensors' access to web applications.
%
We mentioned in the threat model that native iOS applications can still access the motion sensors by default.
%
A new attack scenario is added to evaluation, which considers a real-world scenario where the victim uses the Pencil to write a text message in a chatting application (See \textbf{[MR3]}). 
%
We also detailed how the attacker could train a writing behavior model with a small number of users.
%
We emphasized that this training does not rely on any data collected from the target victim users.
%
Furthermore, we described the details of the data collected for generating the magnetic map as well as the writing behavior model in Section~\ref{sec:data_collection}.
%%

\vspace{2mm}\noindent\textbf{MR6: Details on parameter usage (R4).}
%

We added details on the usage of different parameters in our system in Section~\ref{sec:system_design}.  The parameters that we detailed include, (1) regularization parameters, (2) altitude, azimuth, and rotation ranges, (3) the number of particles, (4) the number of words, and (5) ML model details.

\vspace{1mm}\noindent\textbf{Regularization parameters:} We explained that we perform a grid search for the optimal values of $\lambda_c$ and $\lambda_d$ using the values given in \cite{tafti2011vector} to specify the range for the search.
%
Once the Pencil's magnetic map is generated, their values do not change with the amount of the magnetic samples collected from the victims since the regularization parameters are only needed for magnetic map optimization.

\vspace{1mm}\noindent\textbf{Altitude, azimuth and rotation ranges:} We mentioned in Section~\ref{sec:pencil_tracking} that the ranges for these angles are set based on the minimum and maximum values for these angles observed in the data collected from the attacker for training the writing behavior model.
%
We show in our evaluation that these constraints do not affect our system's performance across different subjects.

%Habiba: need help with this
\vspace{1mm}\noindent\textbf{Number of particles:} We have added explanation in Section~\ref{sec:pencil_tracking} that we perform a grid search to determine the initial number of particles that are sufficient to track the Pencil movement accurately.
%
We generate candidates from a grid of parameter values specified from $10000$ to $10000000$ with increasing the number of particles by $10000$ in each iteration. 
%
We evaluate each of these particle values on the users’ data and use the parameter that leads to highest accuracy at the elbow point~\cite{bishop2006pattern} to prevent overfitting. 
%
Based on our search results, we set the number of particles,$N$, to $5000000$ initially.


\vspace{1mm}\noindent\textbf{Number of words:} We conducted additional experiments to evaluate \sys{}'s performance in detecting words. 
%
We invited $5$ volunteers to write $30$ words each ($150$ words in total), randomly selected from the top $500$ most common English words.
%
We observed that these most common English words vary in length (three - eight letters), complexity, and patterns.
%
In addition to these words, we also conducted experiments where subjects were asked to write three to six lettered words where each letter in the word was chosen randomly from the English alphabet.
%
The purpose of these experiments was to demonstrate \sys{}'s ability to track words in the wild.

\vspace{1mm}\noindent\textbf{ML Model parameters:} We detail the parameters of the models that we use to compare with our \sys{}.
%
The models and their parameters are detailed in the Appendix.




